Hook length biases for self-conjugate partitions and partitions with distinct odd parts

We establish a hook length bias between self-conjugate partitions and partitions of distinct odd parts, demonstrating that there are more hooks of fixed length $t \geq 2$ among self-conjugate partitions of $n$ than among partitions of distinct odd parts of $n$ for sufficiently large $n$. More precisely, we derive asymptotic formulas for the total number of hooks of fixed length $t$ in both classes. This resolves a conjecture of Ballantine, Burson, Craig, Folsom, and Wen.

==> preamble.tex <==
%-------Packages---------
\usepackage{amssymb,amsfonts,mathtools}
\usepackage[all,arc]{xy}
\usepackage{enumerate}
\usepackage{mathrsfs}
\usepackage{amsmath}
\usepackage{hyperref}
\usepackage{amsthm}
\usepackage{tikz}
\usepackage{tikz-cd}
\usepackage[utf8]{inputenc}
\usepackage{lipsum}
\usepackage{extpfeil}
\usepackage{colonequals}
\usepackage{graphicx}
\usepackage{subfig}
\usepackage{enumitem}
\usepackage{array}

%--------Theorem Environments--------
%theoremstyle{plain} --- default
\newtheorem{thm}{Theorem}[section]
\newtheorem{cor}[thm]{Corollary}
\newtheorem{prop}[thm]{Proposition}
\newtheorem{lem}[thm]{Lemma}
\newtheorem{conj}{Conjecture}[section]
\newtheorem*{quest}{Question}
\newtheorem{proper}{Property}[section]
\newtheorem{claim}{Claim}[section]
\newtheorem{ax}{Axiom}[section]
\newtheorem{sta}{Statement}[section]
\newtheorem{fact}{Fact}[section]

\theoremstyle{definition}
\newtheorem{defn}[thm]{Definition}
\newtheorem{defns}[thm]{Definitions}
\newtheorem*{exmp}{Example}
\newtheorem*{exmps}{Examples}
\newtheorem{alg}{Algorithm}
\newtheorem{con}{Construction}[section]
\newtheorem{notn}{Notation}[section]
\newtheorem{notns}{notation}[section]

\theoremstyle{remark}
\newtheorem*{rmk}{Remark}
\newtheorem*{rmks}{Remarks}
\newtheorem{warn}{Warning}[section]
\newtheorem{sch}{Scholium}[section]
\newtheorem{obs}{Observation}[section]
\newtheorem{ass}{Assumption}[section]
\newtheorem{asses}{Assumptions}[section]

\newcommand{\binomd}[2]{\left(\begin{matrix}#1\\ #2 \end{matrix}\right)}

\DeclareMathOperator{\Ob}{Ob}
\DeclareMathOperator{\Mor}{Mor}
\DeclareMathOperator{\id}{id}
\DeclareMathOperator{\RR}{\mathbb{R}}
\DeclareMathOperator{\ZZ}{\mathbb{Z}}
\DeclareMathOperator{\QQ}{\mathbb{Q}}
\DeclareMathOperator{\NN}{\mathbb{N}}
\DeclareMathOperator{\CC}{\mathbb{C}}
\DeclareMathOperator{\FF}{\mathbb{F}}
\DeclareMathOperator{\bbA}{\mathbb{A}}
\DeclareMathOperator{\OO}{\mathcal{O}}
\DeclareMathOperator{\Aut}{\operatorname{Aut}}
\DeclareMathOperator{\Gal}{\operatorname{Gal}}
\DeclareMathOperator{\Hom}{\operatorname{Hom}}
\DeclareMathOperator{\tr}{\operatorname{tr}}
\DeclareMathOperator{\Tr}{\operatorname{Tr}}
\DeclareMathOperator{\pp}{\mathfrak{p}}
\DeclareMathOperator{\qq}{\mathfrak{q}}
\DeclareMathOperator{\disc}{disc}
\DeclareMathOperator{\SL}{\mathrm{SL}}
\DeclareMathOperator{\GL}{\mathrm{GL}}
\DeclareMathOperator{\Div}{\mathrm{Div}}
\DeclareMathOperator{\divis}{\mathrm{div}}
\DeclareMathOperator{\ord}{\mathrm{ord}}
\DeclareMathOperator{\Pic}{\mathrm{Pic}}


\newcommand{\card}[1]{\# #1}
%\newcommand{\card}[1]{\left| #1\right|}


\bibliographystyle{plain}
